Spanning trees in random graphs

For each $\Delta>0$, we prove that there exists some $C=C(\Delta)$ for which the binomial random graph $G(n,C\log n/n)$ almost surely contains a copy of every tree with $n$ vertices and maximum degree at most $\Delta$. In doing so, we confirm a conjecture by Kahn.

==> 1intro.tex <==
The appearance of a Hamilton cycle in the binomial random graph $\GG(n,p)$ is well understood. P\'osa~\cite{posa76} and Korshunov~\cite{kor76} independently proved that, if $p=C\log n/ n$, for some large constant $C>0$, then $\GG(n,p)$ almost surely contains a Hamilton cycle. Koml\'os and Szem\'eredi~\cite{KS83} and Bollob\'as~\cite{bollo83} independently refined the probability required, before Bollob\'as~\cite{bollo84} showed that, in the random graph process, the very edge that is added to cause the graph to have minimum degree two almost surely creates a Hamilton cycle. 

Which other subgraphs may we reasonably expect to appear in the random graph when $p= C\log n/ n$, for some large constant $C$?
We do not expect many short cycles in $\GG(n,p)$, for such a probability $p$, and subgraphs containing vertices with high degree are unlikely to appear. The following conjecture, made by Kahn around twenty years ago~\cite{KK07,KLW14a}, therefore, is natural.
\begin{conjecture}\label{conj}
For every $\Delta>0$, there is some constant $C$ such that, if $T$ is a tree on $n$ vertices with maximum degree at most $\Delta$, then the random graph $\GG(n,C\log n/ n)$ almost surely\footnote{More formally, given any sequence of such trees $(T_n)$, with $|T_n|=n$, $\P(T_n\subset \GG(n,C\log n/ n))\to 1$.} contains a copy of $T$.
\end{conjecture}
If true, this conjecture would be best possible up to the constant $C$, as the random graph involved must almost surely be connected, otherwise it will contain no trees with $n$ vertices. We say such trees \emph{span} the parent graph.

Alon, Krivelevich and Sudakov~\cite{AKS07} studied the related problem of embedding almost-spanning bounded degree trees in a random graph. They showed that, for sufficiently large $c=c(\e,\Delta)$, the random graph $\GG(n,c/n)$ almost surely contains every tree with at most $(1-\e)n$ vertices and maximum degree at most $\Delta$. This is best possible up to the constant $c$, and almost surely finds every such tree simultaneously in $\GG(n,c/n)$. We say that the random graph $\GG(n,c/n)$ is, almost surely, \emph{universal} for this class of trees. Improved bounds for the constant $c(\e,\Delta)$ were found by Balogh, Csaba, Pei and Samotij~\cite{BCPS10}, and the author~\cite{selflove3}, and a resilience version of the result was obtained by Balogh, Csaba and Samotij~\cite{BCS11}.

Let $\TT(n,\Delta)$ be the class of trees which have $n$ vertices and maximum degree at most $\Delta$. When $T\in \TT(n,\Delta)$, Krivelevich~\cite{MK10} showed that, for any $\e>0$, almost surely, the random graph $\GG(n,\max\{(40/\e)\Delta\log n,n^\e\}/n)$ contains a copy of $T$. When $\Delta=n^{\Theta(1)}$ this result is essentially tight, but for smaller $\Delta$ the situation is less clear. For example, where $\Delta$ is constant, this leaves a large gap to Conjecture~\ref{conj}.

Conjecture~\ref{conj} was also studied in particular cases. Clearly, the conjecture is true for the path with $n$ vertices by the results of P\'osa and Korshunov. 

A particular tree, known as the comb, attracted particular interest, as, roughly speaking, it interpolates between these two cases. The \emph{comb} consists of a path $P$ with length $\sqrt{n}-1$ and $\sqrt{n}$ disjoint paths, each starting from a different vertex of $P$ and having length $\sqrt{n}-1$. Conjecture~\ref{conj} was recently confirmed for the comb by Kahn, Lubetzky and Wormald~\cite{KLW14a,KLW14b}, before the author used independent methods to reduce the constant involved as far as possible, showing that we may take $C=1+o(1)$~\cite{selflove3}.


Conjecture~\ref{conj} only seeks a non-universal result. At what probability $p$ can we expect the random graph $\GG(n,p)$ to contain a copy of every tree in $\TT(n,\Delta)$? Johannsen, Krivelevich and Samotij~\cite{JKS12} showed that there is some constant $C>0$ for which, if $\Delta\geq \log n$ and $p\geq C\Delta n^{-1/3}\log n$, then $\GG(n,p)$ is almost surely $\TT(n,\Delta)$-universal. Ferber, Nenadov and Peter~\cite{FNP13} recently showed that $p=\omega(\Delta^8 n^{-1/2}\log^2 n)$ is also sufficient for this to hold, improving the result when $\Delta$ is small.

In this paper we concentrate on the case where $\Delta$ is constant, where these results require an additional factor of $\omega(n^{1/2})$ in the necessary bounds on the probability.
\begin{theorem}\label{unithres}
For every $\Delta>0$, there is a constant $C$ so that, almost surely, the random graph $\GG(n,C\log n/ n)$ contains a copy of every tree with $n$ vertices and maximum degree at most $\Delta$.
\end{theorem}

For each $\Delta>0$, Theorem~\ref{unithres} determines the threshold for the random graph $\GG(n,p)$ to be $\TT(n,\Delta)$-universal, in the process confirming Conjecture~\ref{conj}. The methods used for the proof also work when $\Delta$ is non-constant, giving a marked improvement on what is known when $\Delta$ is small. The dependence of the constant $C$ on $\Delta$ is unlikely to be correct, however, and what this dependence is remains an interesting open question. In the non-universal case, with more work we can find the correct dependence on $\Delta$. This requires however, in addition to the work here, several additional constructions that are largely self-contained, and we defer these to another paper~\cite{selflove5}.

%It is perhaps instructive to briefly recap the methods of the previous best general progress towards the threshold for bounded degree spanning trees. The key observation is that trees is a tree does not have many leaves then it must have in comparison many bare 
%The basic idea here which alone allows us to dramatically reduce the probability required is a variation on a technique call absorption, first outlined as a general method by Rodl, Rucinski and Szemeredi. This allows us to deal with bare paths

Krivelevich~\cite{MK10} observed that if a tree has few leaves then it must, in compensation, contain many long bare paths. In particular, for each $k$, a tree with $n$ vertices must have  at least $n/4k$ leaves or at least $n/4k$ disjoint bare paths with length $k$. Spanning trees with many leaves may be embedded simultaneously and precisely using work by Glebov, Johanssen and Krivelevich~\cite{RomanPhD,GJK14}, as mentioned above.
This reduces the problem to embedding trees in which we can find lots of bare paths. 

In the non-universal case, Krivelevich~\cite{MK10} embedded trees with many bare paths by removing, for constant $k$, $n/4k$ bare paths with length $k$ and embedding the resulting forest into the random graph using results for almost-spanning trees. Revealing more edges in the random graph, it is possible to cover the remaining vertices by paths with length $k$ that replace the removed paths, using a modification of the very strong results by Johansson, Kahn and Vu~\cite{JKV08} on factors in random graphs.

The most important idea in this paper is to embed the trees with lots of bare paths using a version of \emph{absorption}, introduced as a general method by R\"odl, Ruci\'nski and Szemer\'edi~\cite{RRS08}. In their terminology, we use a natural construction for \emph{absorbers}, similar in spirit to that used elsewhere by K\"uhn and Osthus~\cite{KO12} and Allen, B\"{o}ttcher, Kohayakawa and Person~\cite{ABKP13}. Our methods differ from previous implementations in using a system of paths, rather than a single long path, to create the \emph{reservoir} from the absorbers, while achieving this in a comparatively sparse graph.
Using absorption in this way, and relying on the work by Glebov, Johanssen and Krivelevich~\cite{GJK14} would allow us, with an appropriate embedding, to almost surely find the trees under scrutiny in the random graph $\GG(n,\log^2 n/n)$. However, many more ideas and developments are needed to reduce the edge probability to $C\log n/n$, for some large constant $C=C(\Delta)$, particularly as we wish to prove a universal result.

The rest of this paper proves Theorem~\ref{unithres}. In Section~\ref{1boutline} we divide the proof of Theorem~\ref{unithres} into cases before giving an outline of both the proof and the rest of the paper.

We will commonly omit rounding symbols when they are not crucial, and use $\log$ for the natural logarithm. We make little effort to optimize the constant $C(\Delta)$ we produce, as doing so would produce a constant that is not plausibly best-possible.


\subsection{Notation}\label{intronot}

\input{Sections/generalnotation}







==> 2tools.tex <==
\subsection{Notation}
%Note to self, be careful about Glebov et al's definition and use of $N_G(X)$ containing $X$.
A graph $G$ has vertex set $V(G)$, edge set $E(G)$, size $|G|=|V(G)|$ and maximum degree $\Delta(G)$. For the subset $U\subset V(G)$, $G[U]$ is the subgraph of $G$ induced on the set $U$. The set of neighbours of a vertex $v$ is denoted by $N(v)$, and we use $d(v)=|N(v)|$ for the degree of a vertex. Where $U\subset V(G)$, we set $N(v,U)=N(v)\cap U$ to be the neighbours of $v$ in $U$. Where $U\subset V(G)$, we set $N(U)=(\cup_{v\in U}N(v))\setminus U$ and $N'(U)=\cup_{v\in U}N(v)$. We use further notation that naturally extends this, such as $N(U,W)=N(U)\cap W$, without further description. Where there are multiple graphs on the same vertex set we indicate which graph is being considered in the subscript, for example using $d_G(v)$.

Given two subgraphs $H_1,H_2\subset G$, we say that $H_1\cup H_2$ is the subgraph of $G$ with vertex set $V(H_1)\cup V(H_2)$ and edge set $E(H_1)\cup E(H_2)$. Where $P\subset G$ is a path and $H\subset G$ is disjoint from $P$ except for one endvertex of $P$, we think of the graph $H\cup P$ as $H$ with the path $P$ added and let $H+P=H\cup P$. When $xy$ is an edge of a graph $G$ and $H\subset G$, we use $H+e$ for the graph with vertex set $V(H)\cup\{x,y\}$ and edge set $E(H)\cup\{xy\}$.

Given two disjoint vertex sets $A$ and $B$, a \emph{$d$-matching from $A$ into $B$} is a collection of disjoint sets $\{X_a\subset N(a,B):a\in A\}$ so that, for each $a\in A$, $|X_a|=d$. As is well known, such matchings can be found by showing that Hall's generalised matching condition holds. For details on this, and other standard notation, see Bollob\'as~\cite{bollo1}. 



\subsection{Embedding trees and $(d,m)$-extendability}\label{johannsen}
Friedman and Pippenger~\cite{FP87} showed that trees can be found in graphs with certain natural expansion conditions. These expansion conditions, however, require the graph to have many more vertices than the tree. Their method was developed by Haxell~\cite{PH01} to give a general theorem for embedding trees in graphs with certain expansion conditions, which in some cases allow the tree $T$ to have almost as many vertices as the graph. This theorem was used by Balogh, Csaba, Pei and Samotij~\cite{BCPS10} to improve the constant required in the almost-spanning result by Alon, Krivelevich and Sudakov~\cite{AKS07}, as mentioned in Section~\ref{1intro}.

Glebov, Johannsen and Krivelevich~\cite{GJK14} modified Haxell's method to develop a very flexible approach for embedding bounded degree trees. The key definition is that of a \emph{$(d,m)$-extendable subgraph}. Given part of an embedding of a tree which has maximum degree $d$, if it is $(d,m)$-extendable then subject to certain conditions we can add a further vertex of the tree so that the subgraph remains $(d,m)$-extendable. This allows us to build up a copy of the full tree vertex-by-vertex.

\de
Let $d,m\in \N$ satisfy $m\geq 1$ and $d\geq 3$, let $G$ be a graph, and let $S\subset G$ be a subgraph of $G$. We say that $S$ is \emph{$(d,m)$-extendable} if $S$ has maximum degree at most $d$ and
\[
|N'(X)\setminus V(S)|\geq(d-1)|X|-\sum_{x\in X\cap V(S)}(d(x,S)-1)
\]
for all sets $X\subset V(G)$ with $|X|\leq 2m$.
\fn
Note that this definition uses $N'(X)$, the neighbourhood which potentially includes vertices of $X$. We will mostly use the external neighbourhood, $N(X)$, noting that $|N'(X)|\geq |N(X)|$ holds for any vertex set $X$ of any graph, and only turn to $N'(X)$ when deducing properties from the $(d,m)$-extendability of a subgraph.

The following lemma by Glebov, Johannsen and Krivelevich~\cite{GJK14} gives conditions under which a $(d,m)$-extendable subgraph can be extended yet remain $(d,m)$-extendable.
%subgraph shows that under certain conditions a $(d,m)$-extendable subgraph $S$ can have a leaf added to any vertex with degree strictly less then $d$, so that the resulting subgraph remains $(d,m)$-extendable. This allows us, by repeated attachment of leaves, to build up from a single $(d,m)$-extendable vertex any chosen spanning tree.

\lem\label{extendablevertex} Let $d,m\in \N$ satisfy $m\geq 1$ and $d\geq 3$, let $G$ be a graph, and let $S$ be a $(d,m)$-extendable subgraph of $G$. Suppose $G$ satisfies
\begin{equation}\label{crucial}
|N(X)|\geq |V(S)|+2dm+1
\end{equation}
for all subsets $X\subset V(G)$ with $m\leq |X|\leq 2m$. Then, for every vertex $s\in V(S)$ with $d(s,S)\leq d-1$, there exists a vertex $y\in N_G(s)\setminus V(S)$ such that the graph $S+sy$ is $(d,m)$-extendable.
\ma

If we have a $(d,m)$-extendable subgraph $S$ which is a copy of a subgraph of a tree $T$, if $T$ has maximum degree at most $d$, and if the condition with (\ref{crucial}) holds with $S$ replaced by $T$, then Lemma~\ref{extendablevertex} can be used repeatedly to add leaves to $S$ and extend it to a $(d,m)$-extendable copy of $T$. 
%In order to concentrate on other parts of the proof we will not explain this in detail each time, and therefore the following lemma is proved carefully as an example. 
%Note that the proof of Lemma~\ref{almostmethod} does not use the fact that $S$ and $T$ are trees, beyond requiring that we can make $S$ into $T$ by adding a sequence of vertices with degree 1.
As shown by Glebov, Johannsen and Krivelevich~\cite{GJK14}, removing a leaf from, or adding an edge between two vertices with degree at most $d-1$ in, a $(d,m)$-extendable subgraph maintains the extendability, as follows.
\lem\label{extendreverse} Let $d,m\in\N$ satisfy $m \geq 1$ and $d \geq 3$, let $G$ be a graph,
and let $S$ be a subgraph of $G$. Furthermore, suppose there exist vertices $s \in V (S)$ and
$y \in N_G (S) \setminus V (S)$ so that the graph $S+ys$ is $(d, m)$-extendable.
Then $S$ is $(d, m)$-extendable.
\ma
\lem\label{edgeinsert} Let $d,m\in\N$ satisfy $m\geq 1$ and $d\geq 3$, let $G$ be a graph, and let $S$ be a $(d,m)$-extendable subgraph of $G$. If $s,t\in V(S)$ with $d_S(s),d_S(t)\leq d-1$ and $st\in E(G)$, then $S+st$ is a $(d,m)$-extendable subgraph of $G$.
\ma

In addition, Glebov, Johannsen and Krivelevich~\cite{GJK14} proved the following connection lemma, which allows a path to be added to a $(d,m)$-extendable subgraph while keeping the extendability. We record a slightly stronger statement in Lemma~\ref{extendableconnect} than which can be found in~\cite{GJK14}, but it follows with an identical proof.

\lem\label{extendableconnect} Let $n,d,m\in\N$ satisfy $m\geq 1$ and $d\geq 3$, let $G$ be a graph on $n$ vertices satisfying $e_G(X,Y)> 1$, for all disjoint sets $X,Y\subset V(G)$ with $|X|\geq m$ and $|Y|\geq m$, and let $S$ be a $(d,m)$-extendable subgraph of $G$ with at most $n-10dm$ vertices. 

Let $k=\lceil\log (2m)/ \log(d-1)\rceil$ and let $j\in\{1,\ldots,k\}$. Suppose there are two disjoint vertex sets $A$ and $B$ in $S$, each with size at least $2m/(d-1)^j$, so that all the vertices in $A$ and $B$ have degree at most $d/2$ in $S$. Then there exist two disjoint paths $P_1$ and $P_2$ with length $j$ in $G$ and contains the endvertices $a\in V(P_1)$ and $b\in V(P_2)$ in $A$ and $B$ respectively such that all the vertices of $P$ except $a$ or $b$ are not in $S$, there is an edge between the two endpoints not in $A$ or $B$, and $S+P_1+P_2$ is $(d,m)$-extendable.
\ma

Lemma~\ref{edgeinsert} allows us to add a path with length $2j+1$ between the sets $A$ and $B$ in the above lemma, while keeping the extendability, by adding the edge $ab$ to the subgraph. Note that, in Lemma~\ref{extendableconnect}, a path of length $2k+1$ can be added between any two vertices of the subgraph with degree at most $d/2$. Therefore, with the same conditions as in Lemma~\ref{extendableconnect}, if $S$ has at most $n-10dm-l$ vertices, then we can add a path with length $2k+l+1$ between any two vertices $x$ and $y$ if they each have degree at most $d/2$ in $S$. Indeed, using Lemma~\ref{extendablevertex} repeatedly, we can attach a path with length $l$ to $x$ and by Lemma~\ref{extendableconnect} we can find a path with length $2k+1$ between the end of that path and $y$, all while maintaining the $(d,m)$-extendability.

In combination, Lemmas~\ref{extendableconnect},~\ref{extendreverse},~\ref{edgeinsert} and~\ref{extendablevertex} provide a very flexible framework for manipulating almost-spanning trees as we embed them into our graph. To help us move between Lemma~\ref{extendableconnect} and Lemma~\ref{extendablevertex}, note that if there is some edge between any two $m$ sets in a graph and $U\subset V(G)$ with $m\leq |U|\leq 2m$, then as there are no edges between $U$ and $V(G)\setminus (N(U)\cup U)$, we must have $|N(U)|\geq n-3m$. Therefore, if the conditions in 
For every vertex set $U\subset V(G)\setminus X_2$ with $m\leq |U|\leq 2m$ we know that $|N(U)|\geq n-|X_2|-|U|-m\geq n-9m\geq n-|L|+10\Delta m=|T'|+10\Delta m$. Therefore, if the conditions in the first paragraph of Lemma~\ref{extendableconnect} hold for a subgraph $S$ and graph $G$, then we can apply Lemma~\ref{extendablevertex} to that subgraph.


%In combination, Lemmas~\ref{extendablevertex} and~\ref{extendableconnect} form a flexible framework for embedding a tree $T$ into a graph $G$ as long as we have an extra $10dm$ vertices to work with.
%We will want the following variation of Lemma~\ref{extendableconnect}. Lemma~\ref{extendableconnect2} can be proved almost identically to Lemma~\ref{extendableconnect} so we will not go into details. As the conditions in Lemma~\ref{extendableconnect2} are very similar to those in Lemma~\ref{extendablevertex} it is easy to use them together.
%\lem\label{extendableconnect2}  Let $n,d,m\in\N$ satisfy $m\geq 1$, $d\geq 3$ and $1000dm\leq n$. Let $G$ be a graph on $n$ vertices satsifying $|N(X)\geq (1-1/100)n$ for all sets $X\subset V(G)$ with $m\leq |X|\geq 2m$, and let $S$ be a $(d,m)$-extendable subgraph of $G$ on at most $n/2$ vertices. Let $k=\lceil\log (2n)/ \log(d-1)\rceil$ and let $j\in\{1,\ldots,k\}$. Assume that there are two disjoint vertex sets $A$ and $B$ in $S$ such that both $A$ and $B$ are of size at least $2n/(d-1)^j$ and all vertices in $A$ and $B$ are of degree at most $d/2$ in $S$. Then there exists a path $P$ of length $j+1$ in $G$ with endpoints in $A$ and $B$ such that all vertices of $P$ except the two endpoints do not belong to $S$, and $S+P$ is $(d,m)$-extendable.
%\ma






\subsection{Properties of the random graph $\GG(n,p)$}
We recall here some standard facts concerning the random graph. Due to the remarks in Section~\ref{almostsure}, some of the lemmas we use will be far from optimal to make sure the properties involved are particularly likely to hold. The following three simple proposition follow using simple probabilistic calculations or Chernoff bounds.

\begin{prop}\label{alledges} Suppose $p=\omega(1/n^2)$. Then the random graph $\GG(n,p)$ almost surely has between $pn^2/4$ and $pn^2$ edges.
\end{prop}

\begin{prop}[Alon, Krivelevich and Sudakov~\cite{AKS07}, Proposition 3.2]\label{AKS1}
Let $G=\GG(n,p)$ be a random graph with $np>20$. Then almost surely the number of edges between any two disjoint subsets of vertices $A$, $|A|=a$, and $B$, $|B|=b$, with $abp\geq 32n$ is at least $abp/2$ and at most $3abp/2$.
\end{prop}

\begin{prop}[\cite{selflove3}]\label{generalprops} If $np>20$, then almost surely any two disjoint vertex sets $A$ and $B$ of $G=\GG(n,p)$ with $|A|,|B|\geq 5\log(np)/ p$ have some edge between them.
\end{prop}

Note, as will be useful, an immediate corollary of Proposition~\ref{generalprops} is that under these conditions almost surely any two sets with size at least $10\log(np)/p$ have at least two edges between them.

It will also be convenient to use the following result by Vu~\cite{Vu01} on the number of subgraphs of a random graph  isomorphic to some fixed balanced subgraph $H$ (a balanced subgraph is one whose density, calculated as $|E(H)|/|V(H)|$, is at least as large as the density of any subgraph). Theorem~\ref{subcount} records the part of Theorem 1.1 in \cite{Vu01}  we wish to use, and Corollary~\ref{fewpathslengthtwo} confirms the specific case we need.
\begin{theorem}\label{subcount}
Let $0<\e\leq 1$. Suppose $H$ is a balanced graph with $k$ vertices, and $Y$ is the random variable counting the number of subgraphs of a random graph $\GG(n,p)$ isomorphic to $H$. Suppose further that $\e^2(\E Y)^{1/(k-1)}=\omega(\log n)$. Then there is a positive constant $c=c(H)$ such that
\[
\P(Y\geq (1+\e)\mathbb{E} Y)\leq \exp(-c\e^2(\mathbb{E}Y^{1/(k-1)})).
\]
\end{theorem}
\begin{corollary}\label{fewpathslengthtwo}
Suppose $n^3p^2=\omega(\log^2 n)$, then almost surely $\GG(n,p)$ contains at most $n^3p^2$ paths with length two.
\end{corollary}
\ifdraft
\else
\pr
Let $P$ be the path with length two and let $Y$ be the number of subgraphs of $\GG(n,p)$ which are isomorphic to $P$. Then $(\mathbb{E}Y)^{1/2}=(3\binom{n}{3}p^2))^{1/2}=\omega(\log n)$. As $P$ is balanced, by Theorem~\ref{subcount} with $\e=1$, $\P(Y\geq 6\binom{n}{3}p^2)\leq n^{-\omega(1)}$. 
\oof
\fi

\subsection{Expansion and Matchings}
Finding matchings is a crucial tool for attaching leaves to trees, and matchings can be found from expansion conditions by showing Hall's matching condition holds, as follows.

\lem\label{matchings} Let $n,m\in \N$. Suppose $H$ is a bipartite graph with vertex classes $A$ and $B$, where $|A|=|B|=n$ and the following holds. For all sets $U\subset A$ or $U\subset B$, if $|U|<m$, then $|N(U)|\geq |U|$ and if two sets $U\subset A$ and $U'\subset B$ each have $m$ vertices, then there is some edge between them. Then there is a matching between $A$ and $B$.
\ma
\ifdraft
\else
\pr We will demonstrate Hall's matching condition holds between $A$ and $B$. Suppose $U\subset A$. If $|U|< m$, then $|N(U)|\geq |U|$. 

If $m\leq |U|\leq n-m$, then, as there are no edges between $U$ and $B\setminus N(U)$, we must have that $|B\setminus N(U)|< m$. Thus, $|N(U)|\geq |B|-|B\setminus N(U)|> n-m\geq |U|$.

If $|U|\geq \max\{n-m,m\}$, then by the same reasoning as above, $|N(U)|> n-m$. Therefore, $|B\setminus N(U)|< m$, and hence $|N(B\setminus N(U))|\geq |B\setminus N(U)|$. However, $N(B\setminus N(U))$ and $U$ are disjoint sets in $A$, so $|B\setminus N(U)|+|U|\leq n$. Therefore, $|N(U)|\geq |U|$, and Hall's matching condition holds between $A$ and $B$.
\oof
\fi

We also will use the following lemma on $d$-matchings in the random graph.
\lem\label{logmatching}
Let $A$ and $W$ be fixed disjoint vertex subsets of the random graph $\GG(n,p)$, where $p|W|\geq 25\log n$, and suppose $1\leq d\leq p|W|/4$ and $|A|\leq |W|/2d$. Then, almost surely, there is a $d$-matching from $A$ into $W$. 
\ma
\pr Let $l=|A|$ and label the vertices in $A$ as $a_1,\ldots,a_l$. Let $W_0=\emptyset$. Reveal the edges adjacent to each vertex $a_i$ of $\GG(n,p)$ in turn. At each reveal, if it is possible to find $d$ neighbours of $a_i$ in $W\setminus W_{i-1}$, then do so, adding them to $W_{i-1}$ to get $W_i$. The probability this is not possible for a fixed vertex $a_i$ will be at most $\P(\mathrm{Bin}(|W|-d(i-1),p)\leq d)\leq \P(\mathrm{Bin}(|W|/2,p)\leq p|W|/4)\leq 2\exp(-p|W|/8)=o(n^{-3})$, using a Chernoff bound. Therefore, the probability this process fails to find a $d$-matching from $A$ into $W$ is at most $o(n^{-2})$.
%Given any subset $U\subset A$, with $|U|=k$, the probability $q_k$ vertex $x\in W$ is in $N(U,W)$ is $1-(1-p)^{k}$. If $pk\leq 1/2$, then this is at least $pk/2$. If $pk\geq 1/2$, then $q_k\geq 1-e^{-pk/2}\geq
\oof
We will often wish to find certain expansion properties by revealing edges in a random graph, and the following lemma covers all the cases we will need. The following proof could also be proved using a more direct calculation, but we take the opportunity to use a simple but effective technique that is used throughout this paper. It finds expansion properties in a subset of the random graph by removing a set subject to certain conditions.

\lem\label{generalexpand} Let $W\subset V(G)$ be a fixed subset of the random graph $G=\GG(n,p)$ with $p|W|\geq 100\log n$. Let $m=20\log(np)/ p$ and $d$ satisfy $2\leq d\leq |W|/12m\geq 1$. Then, almost surely, we have that any subset $U\subset V(G)$ with $|U|\leq |W|/12d$ satisfies $|N(U,W)|\geq d|U|$.
\ma
\pr Reveal edges with probability $p/2$. Almost surely, by Proposition~\ref{generalprops}, any two disjoint sets of size at least $m$ must have some edge between them. Let $B\subset V(G)$ be a maximal subset subject to the conditions $|B|\leq m$ and $|N(B,W)|< 3d|B|$. Take any subset $U\subset V(G)\setminus B$ with $|U|\leq |W|/12d$, and suppose that $|N(U,W\setminus B)|<3d|U|$. Then $|N(B\cup U,W)|< 3d(|B|+|U|)$, so, by the definition of $B$, $|B\cup U|\geq m$. There are no edges between $B\cup U$ and $W\setminus (B\cup U\cup N(B\cup U))$, so $|W\setminus (B\cup U\cup N(B\cup U))|\leq m$. Therefore,
\[
|N(U,W\setminus B)|\geq |W|-m-|B|-|U|-3d|U|\geq |W|/4\geq 3d|U|.
\]
Reveal more edges with probability $p/2$ between $B$ and $W\setminus B$ to complete the random graph $G$, in which each edge has been revealed with probability at most $p$. Almost surely, we have by Lemma~\ref{logmatching} a $2d$-matching from $B$ into $W\setminus B$. Given $U\subset V(G)$, with $|U|\leq m$, and noting either $|U\cap B|\geq |U|/2$ or $|U\setminus B|\geq |U|/2$, we have
\[
|N(U,W)|\geq \max\{|N(U\cap B,W)|,|N(U\setminus B,W)|\}-|U|\geq 3d(|U|/2)-|U|\geq d|U|.\qedhere
\]
\oof
The following lemma can be proved using similar calculations as above, but is a consequence of the value of the threshold for a bipartite graph containing a matching (see Bollob\'as~\cite{bollo1} for details).

\lem\label{matchingthres} Let $H$ be a random bipartite graph with classes $A$ and $B$, with $|A|=|B|=n$, and edges between $A$ and $B$ present independently with probability $10\log n/ n$. Then, almost surely, there is a matching between $A$ and $B$.
\ma

We also need the following result later, which find bipartite graphs with few edges but good expansion properties.
\lem\label{randommatchingsexpand} Let $H$ be a random bipartite graph with classes $X$ and $Y$, $|X|=|Y|=n$, formed by taking 20 random matchings between $X$ and $Y$. Almost surely, the following hold.
\begin{itemize}
\item If $A\subset X$ and $|A|\leq n/4$, then $|N(A)|\geq 2|A|$.
\item If $B\subset Y$ and $|B|\leq n/4$, then $|N(B)|\geq 2|B|$.
\item If $A\subset X$, $B\subset Y$ and $|A|,|B|\geq n/4$, then there is some edge between $A$ and $B$.
\end{itemize}
\ma
\ifdraft
\else
\pr
Given two sets $A\subset X$ and $B\subset Y$, and a random matching $M$ between $X$ and $Y$, the probability that $N_M(A)\subset B$ is $\binom{|B|}{|A|}\binom{n}{|A|}^{-1}$. Thus, for each $t\leq n/4$, the probability there is some set $A\subset X$ with $|A|=t$ and $|N_H(A)|<2t$ is at most
\[
\binom{n}{t}\binom{n}{2t}\left(\binom{2t}{t}\binom{n}{t}^{-1}\right)^{20}
\leq \left(\frac{e^3}{4}\left(\frac nt\right)^{3}\left(\frac{2t}{n}\right)^{20}\right)^t
= \left(2e^3\left(\frac{2t}{n}\right)^{17}\right)^t.
\]
Looking separately at the cases $t\leq \log n$, and $\log n\leq t\leq n/4$, we see that the sum of these probabilities tends to 0 as $n\to\infty$. An identical calculation shows that, almost surely, $|N(B)|\geq 2|B|$ for every $B\subset Y$ with $|B|\leq n/4$.

The probability there are no two sets $A\subset X$ and $B\subset Y$, with $|A|=|B|=\lceil n/4\rceil$ and $e(A,B)=0$ is at most
\[
\binom{n}{n/4}^2\left(\binom{3n/4}{n/4}\binom{n}{n/4}^{-1}\right)^{20}\leq (4e)^{n/2}\left(\frac{3}{4}\right)^{20n/4}\leq \left(\frac12\right)^{n/4}. 
\]
Therefore, almost surely, all three of these properties in the lemma hold.
\oof
\fi

















\subsection{Leaves and bare paths in trees}
The following lemma by Krivelevich~\cite{MK10} shows that trees without many leaves must contain many bare paths in compensation.

\lem\label{Kleaves} Let $k,l,n>0$ be integers. Let $T$ be a tree with $n$ vertices with at most $l$ leaves. Then $T$ contains a collection of at least $n/(k+1)-(2l-2)$ vertex disjoint bare paths with length $k$ each.
\ma
This lemma will be used in the following form, taking $l=n/4k$.

\begin{corollary}\label{split} For any integers $n,k>2$, a tree with $n$ vertices either has at least $n/4k$ leaves or a collection of at least $n/4k$ vertex disjoint bare paths, each with length $k$.
\end{corollary}

When embedding trees, we wish to control where we embed certain vertices. This will be easier if these certain vertices are far apart in the tree. With this in mind, we prove the following lemma.

\lem\label{farleaves}
Let $n,k$ and $d$ be integers with $n\geq 60k$ and $k\geq 4d$. Suppose a tree $T$ with $n$ vertices has at most $n/5d$ leaves. Then $T$ either contains a collection of at least $n/40k$ leaves which are pairwise a distance at least $2d$ apart in $T$ or a collection of $n/40k$ vertex disjoint bare paths with length $k$.
\ma
\ifdraft
\else
\pr
By Corollary~\ref{split}, as $T$ has at most $n/5d$ leaves there are $m=\lceil n/4d\rceil$ vertex disjoint bare paths $P_i$, $i\in[m]$, with length $d$ in $T$. Contract each path $P_i$ to a single edge $e_i$, and contract all the other edges in $T$ which are not in a path $P_i$. The resulting tree, $S$ say, has one edge for each path $P_i$, so $|S|= m+1$. Let $k_0:=\lceil k/d\rceil\leq 5k/4d$. By Corollary~\ref{split}, the tree $S$ either has at least $m/4k_0$ leaves or contains at least $m/4k_0$ vertex disjoint bare paths with length $k_0$. 

If $S$ has at least $m/4k_0\geq n/16dk_0\geq n/20k$ leaves, then let these leaves be the vertices $v_i$, $i\in I$, contained in the edges $e_i$, $i\in I$, with $|I|\geq n/20k$. As $n>60 k$, $|S|\geq 3$, and each edge $e_i$ can contain at most one leaf. For each $i\in I$, consider the tree which was contracted to get the vertex $v_i$, and call it $T_i$. Either $|T_i|=1$, in which case the vertex is unchanged and is a leaf in $T$, which we call $u_i$, or $T_i$ has at least  two leaves, one of which must be a leaf in $T$, which we call $u_i$. If $i\neq j$ then $u_i$ and $u_j$ are separated from each other in the tree by both $P_i$ and $P_j$, so are a distance at least $2d$ apart in $T$ and we have a suitable set of leaves.

Suppose then $S$ has at least $n/20k$ bare paths with length $k_0$, and fix such a set of paths. Take such a path and look at the trees that were contracted together to get each internal vertex. If none of these trees had any leaves in $T$ then the bare path in $S$ came from a bare path with length at least $dk_0\geq k$ in $T$. If this is true for at least $n/40k$ of the paths in $S$ then we have the required number of paths with length $k$. If not, then at least $n/40k$ of the paths have an internal vertex which came from contracting a tree that contains a leaf of $T$. Collecting a leaf like this from each path gives a set of leaves which are pairwise a distance at least $2k_0\geq 2d$ apart in $T$.
%  then take a set of such paths and consider one of them formed from edges $e_i$, $i\in I$. If There is some path in $T$ which contains all the paths $P_i$ - take the shortest such path, $Q$ say. This path must have length at least $15k_0\geq k$, and the paths formed from the distinct paths in $S$ form distinct paths in $T$.
%Either $Q$ is a bare path in $T$, or it is not. If $Q$ is not bare in $T$ then there must be some leaf $l$ branching off that path which is a distance at least 15 from either endpoint of $Q$ in $T$. If $Q$ is bare then it contains a bare path length $k$. If we have the first case for $n/40k$ bare paths in $S$ then by taking one leaf off each path we have at least $n/40k$ leaves at a distance of at least 30 apart. If we have the second case for $n/40k$ bare paths in $S$, then this gives $n/40k$ disjoint bare paths in $T$, each with length at least $k$. 
\oof
\fi
Lemma~\ref{splitclass}, which permits the splitting of Theorem~\ref{unithres} into four cases in Section~\ref{1boutline}, now follows easily.
\pr[Proof of Lemma~\ref{splitclass}] Let $\delta=1/400\Delta^{20}$ and suppose $T\in\TT(n,\Delta)$ has $\lambda(T)\leq \d n$. If $T$ has at least $n/100$ leaves, then, as each leaf has at most $2\Delta^{20}$ vertices within a distance $20$ in $T$, then $\lambda(T)\geq n/200(\Delta^{20}+1)>\d n$, a contradiction. Therefore, $T$ has fewer than $n/100$ leaves, so by Corollary~\ref{split}, $k'(T)\geq 25$. If $k'=k'(T)$, then the tree $T$ does not contain $n/90(k'+1)$ disjoint paths with length $k'+1$, so, by Lemma~\ref{farleaves}, $\l(T)\geq n/90(k'+1)$. Therefore, $k(T)\l(T)\geq n/100$, and thus, for sufficiently large $n$, Case A and B cover all trees $T\in \TT(n,\Delta)$ with $k(T)<10^2\log n$.
\oof

In our embeddings we often want to divide a tree into pieces with different properties. This can by done using the following definition and proposition.

\de
Where $S$ is a tree, we say two subtrees $S_1$ and $S_2$ \emph{divide $S$} if they cover $S$ and intersect on precisely one vertex.
\fn

\begin{prop}[\cite{selflove3}]\label{divide}
Given a tree $S$ with a vertex set $Q\subset V(S)$, we can find two trees $S_1$ and $S_2$ which divide $S$ for which $|V(S_1)\cap Q|, |V(S_2)\cap Q|\geq |Q|/3$.
\end{prop}

In Proposition~\ref{divide}, by taking $Q=V(S)$ we can find two trees which divide $S$ and each contain at least $|S|/3$ vertices. If $S$ has $m$ vertex disjoint bare paths length $k$, then, by taking a vertex from the middle of each of these paths to form $Q$, we can find two trees which divide $S$ and each contain at least $m/3-1$ vertex disjoint bare paths with length $k$.

\begin{prop}\label{littletree} Let $n,m\in \N$ satisfy $1\leq m\leq n/3$. Given any tree $T$ with $n$ vertices and a vertex $t\in V(T)$, we can find two trees $T_1$ and $T_2$ which divide $T$ so that $t\in V(T_1)$ and $m\leq |T_2|\leq 3m$.
\end{prop}
\pr Find trees $T_1$ and $T_2$, with $t\in V(T_1)$, which divide $T$, so that $|T_2|$ is minimized subject to $|T_2|\geq m$. Some pair of trees satisfying these conditions exists by Proposition~\ref{divide}, so this is possible. Suppose $|T_2|>3m\geq 3$. Using Proposition~\ref{divide} find trees $T_3$ and $T_4$ which divide $T_2$ so that $|T_3|,|T_4|\geq \lceil |T_2|/3\rceil\geq 2$. Let $t'=V(T_1)\cap V(T_2)$ and suppose without loss of generality that $t'\in V(T_3)$. Consider the trees $T_5=T_3\cup T_1$ and $T_4$. The tree $T_5$ contains $t$, and $|T_2|>|T_4|\geq |T_2|/3\geq m$, a contradiction. Therefore, $|T_2|\leq 3m$.
\oof


==> spanpic2.tex <==
\begin{figure}
\centering
    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic1A}
        }
    \end{subfigure}\parbox[b]{.4\linewidth}{%
\subcaption{The stage $q$ situation from Figure~\ref{spanpic1}, where $q=8$. The vertices in $X_q\subset X$ are grey, as are the vertices~$z_i$, $i\in I$. Corollary~\ref{extendableconnectcor} is then applied to the sets $\{z_i:i\in I\}$ and $X_q$ to reach the situation in (b).
\\
\textcolor{white}{.}}}

    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic1B}
        }
    \end{subfigure}\parbox[b]{.4\linewidth}{%
\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_2$}. We have found the path~$P_2$ and the edge $e_2\in E(P_2)$, so that $S+P_2-e_2$ is $(d,m)$-extendable and $P_2$ embeds the vertex $q_2$ onto $x_2$. Step~{\bfseries \Alph{capitalcounterbackup}$_2$} is therefore a good step.\\
\textcolor{white}{.}}}

    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic1C}
        }
    \end{subfigure}\parbox[b]{.4\linewidth}{%
\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path~$P_3$ and an edge $e_3$  satisfying the conditions for Step~{\bfseries \Alph{capitalcounterbackup}$_3$} to be a good step. Therefore, we have found instead the path $P_3$, so that $(S+P_2-e_2)+P_3$ is $(d,m)$-extendable. Step~{\bfseries \Alph{capitalcounterbackup}$_3$} is therefore a neutral step.\\
\textcolor{white}{.}}}


    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic1D}
        }
    \end{subfigure}\parbox[b]{.4\linewidth}{%
\subcaption{After the final step, Step~{\bfseries \Alph{capitalcounterbackup}$_q$}, has been completed, when $q=8$.
We have had in total four good steps (Steps~{\bfseries \Alph{capitalcounterbackup}$_2$},~{\bfseries \Alph{capitalcounterbackup}$_4$},~{\bfseries \Alph{capitalcounterbackup}$_6$} and~{\bfseries \Alph{capitalcounterbackup}$_7$}) and three neutral steps (Steps~{\bfseries \Alph{capitalcounterbackup}$_3$},~{\bfseries \Alph{capitalcounterbackup}$_5$} and~{\bfseries \Alph{capitalcounterbackup}$_8$}).\\
\textcolor{white}{.}}}


\caption{An illustration of the proof of Claim~\ref{claimy}.} \label{spanpic1}
\end{figure}



==> spanpic5.tex <==
\begin{figure}[t!]
\centering
    \begin{subfigure}{0.8\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic5A1}
        }
\label{spanpic4A1}
    \end{subfigure}
\begin{comment}
%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3B1}
        }
\label{spanpic3B1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3B2}
        }
\label{spanpic3B2}
    \end{subfigure}


%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3C1}
        }
\label{spanpic3C1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3C2}
        }
\label{spanpic3C2}
    \end{subfigure}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3D1}
        }
\label{spanpic3D1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3D2}
        }
\label{spanpic3D2}
    \end{subfigure}


%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

\end{comment}
\caption{A depiction of Lemma} \label{spanpic1}
\end{figure}



==> spanpic5B.tex <==
\begin{figure}
\centering
    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic5B1}
        }
\label{spanpic4A1}
    \end{subfigure}

\vspace{-0.5cm}











\caption{Continuing with the structure in Figure~\ref{spanpic5A} and with $\a=3$, for each $j\in[\a]$ we pick disjoint pairs $(u_{j,i},v_{j,i})$, $i\in [w_j]$, of vertices from $W_j\setminus A_{j+1}$, and, further disjoint pairs $(u_{\a+1,i},v_{\a+1,i})$, $i\in [r/2-k']$ in $V(G)\setminus (\cup_{i\in [\a+1]}A_i)$. For each $j\in [\a+1]$ typical vertices $u_{j,i}$ and $v_{j,i}$ are labelled in the figure. We let $X$ be the set of all 
these vertices. We relabel these vertices as $(x_i,y_i)$, $i\in [r/2]$, for the statement of the lemma, but use the first labels in Figures~\ref{spanpic5C} and~\ref{spanpic5D}.
We then let $A=\cup_{i\in[\a+1]}A_i$, which, with $X$, will satisfy the requirements of Lemma~\ref{almostspan}.
} \label{spanpic5B}
\end{figure}



==> spanpic5D.tex <==
\begin{figure}[p]
\centering
    \begin{subfigure}[b]{\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic5D1}
        }
\label{spanpic5D1}
    \end{subfigure}

%\vspace{-0.5cm}











\caption{A typical Step~$\mathbf{\Alph{STEPJcounter}}_j$ in the proof of Lemma~\ref{almostalmostspan2}, here shown for $j=3$. We take the cycle $Q_4$, as shown in Figure~\ref{spanpic5C}, and divide it into subpaths with new endvertices giving the pairs $(u'_{j,i},v'_{j,i})$, $i\in [w_j]$. Recalling the set $W_j$ from Figure~\ref{spanpic5A} we see that it contains these new vertices, as well as the vertices $u_{j,i}$, $v_{j,i}$, $i\in [w_j]$. Therefore, we can use Property~\ref{B1} to find the $u_{j,i},v_{j,i}$-paths, $i\in [w_j]$ using vertices from $A_j$ and the vertices in $Q_{j+1}$, while covering the other vertices in $A_j$ by the cycle $Q_j$. The paths found so far then cover $A_{j+1}$, and all of $A_j$ except for the cycle $Q_j$, which we use to start the next step. When all the Steps~$\mathbf{\Alph{capitalcounter}}_j$ from $j=\a$ to $j=1$ have been completed, all of $A=\cup_iA$ will be covered with paths, except for the final cycle $Q_1$, which lies in $A_1$, and hence~$W_0$, as required.  
} \label{spanpic5D}
\end{figure}



==> spanpic6.tex <==
\begin{figure}
\centering
    \begin{subfigure}[b]{1\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic6A1}
        }
\label{spanpic4A1}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            %\input{spanpic5A2}
        }
\label{spanpic4A2}
    \end{subfigure}
\begin{comment}
%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3B1}
        }
\label{spanpic3B1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3B2}
        }
\label{spanpic3B2}
    \end{subfigure}


%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3C1}
        }
\label{spanpic3C1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3C2}
        }
\label{spanpic3C2}
    \end{subfigure}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3D1}
        }
\label{spanpic3D1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3D2}
        }
\label{spanpic3D2}
    \end{subfigure}


%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

\end{comment}
\caption{Important sets found in the random graph $G$ in the proof of Theorem~\ref{unithres} in Case~B, along with the vertex $v_0\in Z_3$. The sets $L_0$, $M$, $Z_3$, $Z_5$, $W_0$ and $X$ partition $V(G)$. As well as keeping the set $Z_4$ in mind, we remember that $Z_3\cup Z_4\subset Z_1$.} \label{spanpic6A}
\end{figure}



==> spanpic7.tex <==
\begin{figure}
\centering
    \begin{subfigure}[b]{1\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic7A1}
        }
\label{spanpic7A1}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            %\input{spanpic5A2}
        }
\label{spanpic4A2}
    \end{subfigure}
\begin{comment}
%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3B1}
        }
\label{spanpic3B1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3B2}
        }
\label{spanpic3B2}
    \end{subfigure}


%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3C1}
        }
\label{spanpic3C1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3C2}
        }
\label{spanpic3C2}
    \end{subfigure}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3D1}
        }
\label{spanpic3D1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3D2}
        }
\label{spanpic3D2}
    \end{subfigure}


%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

\end{comment}
%\caption{A depiction of Lemma} \label{spanpic1}
\end{figure}



==> spanpic7C.tex <==
\begin{figure}[p]
\centering
    \begin{subfigure}[b]{0.7\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic7C7}
        }
\label{spanpic46A1}
    \end{subfigure}

\vspace{-0.5cm}


\caption{On the left, from top to bottom, is the situation in the embedding for a tree $T$ in Case~$B$ immediately after each stage, from Stage 1 to Stage 4. In each picture the sets and trees in black represent a partition of $V(G)$. On the right, from top to bottom, are the subgraphs of $T$ that have been embedded in the matching pictures on the left. The blue arrow in the third picture down on the left represents the vertices in $(U_0\cup Z_3)\setminus V(S_3)$ being moved to form $U_1$.}
\label{spanpic6C}
\end{figure}



==> spanpic82.tex <==
\begin{figure}[b]

\vspace{0.25cm}

\centering
    \begin{subfigure}[b]{0.95\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic8A2}
        }
    \end{subfigure}\label{spanpic8A2}
\begin{comment}
%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3B1}
        }
\label{spanpic3B1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3B2}
        }
\label{spanpic3B2}
    \end{subfigure}


%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3C1}
        }
\label{spanpic3C1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3C2}
        }
\label{spanpic3C2}
    \end{subfigure}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3D1}
        }
\label{spanpic3D1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3D2}
        }
\label{spanpic3D2}
    \end{subfigure}


%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

\end{comment}
\caption{An $x_i,y_i$-path through the absorber $(B_i,x_i,y_i)$ and the vertex~$v_2$ (cf.\  Figure~\ref{spanpic8}). Similarly, we can find $x_i,y_i$-paths through $(B_i,x_i,y_i)$ and either the vertex~$v_1$ or the vertex~$v_3$.} \label{spanpic82}
\end{figure}



==> spanpicH.tex <==
\begin{figure}
\centering
         \input{spanpicH1}
 \label{spanpic4A1}
 
\begin{comment}
%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3B1}
        }
\label{spanpic3B1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3B2}
        }
\label{spanpic3B2}
    \end{subfigure}


%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3C1}
        }
\label{spanpic3C1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3C2}
        }
\label{spanpic3C2}
    \end{subfigure}

    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3D1}
        }
\label{spanpic3D1}
    \end{subfigure}
\hspace{-0.25cm}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \resizebox{\linewidth}{!}{
            \input{spanpic3D2}
        }
\label{spanpic3D2}
    \end{subfigure}


%\subcaption{After Step~{\bfseries \Alph{capitalcounterbackup}$_3$}. We could not find a path $P_2$ satisfying our conditions with an endpoint in we have found the path $P_1$, so that $S\cup S_1+P_1-e_1$ is $(d,m)$-extendable and which embeds a $q_1$ onto $x_1$. Step is therefore a neutral step.}

\end{comment}

\caption{A graph $H$, shown on the left, satisfying the properties stated in Lemma~\ref{flexiblematching} when $h=9$. As depicted on the right, given any subset $Z'\subset Z$ satisfying $|Z'|=h/3$ there is a matching between $X$ and $Y\cup Z'$ in $H$.} \label{spanpic1}
\end{figure}


